MLPerf HPC: A Holistic Benchmark Suite for Scientific Machine Learning on HPC Systems

Scientific communities are increasingly adopting machine learning and deep learning models in their applications to accelerate scientific insights. High performance computing systems are pushing the frontiers of performance with a rich diversity of hardware resources and massive scale-out capabilities. There is a critical need to understand fair and effective benchmarking of machine learning applications that are representative of real-world scientific use cases. MLPerf is a community-driven standard to benchmark machine learning workloads, focusing on end-to-end performance metrics. In this paper, we introduce MLPerf HPC, a benchmark suite of large-scale scientific machine learning training applications driven by the MLCommons Association. We present the results from the first submission round, including a diverse set of some of the world's largest HPC systems. We develop a systematic framework for their joint analysis and compare them in terms of data staging, algorithmic convergence, and compute performance. As a result, we gain a quantitative understanding of optimizations on different subsystems such as staging and on-node loading of data, compute-unit utilization, and communication scheduling, enabling overall $>10 \times$ (end-to-end) performance improvements through system scaling. Notably, our analysis shows a scale-dependent interplay between the dataset size, a system's memory hierarchy, and training convergence that underlines the importance of near-compute storage. To overcome the data-parallel scalability challenge at large batch sizes, we discuss specific learning techniques and hybrid data-and-model parallelism that are effective on large systems. We conclude by characterizing each benchmark with respect to low-level memory, I/O, and network behavior to parameterize extended roofline performance models in future rounds.

==> sources/02_MLPerf.tex <==
\section{MLCommons/MLPerf}


\Murali{merge with section 3}

MLCommons \cite{mlcommons} is an open engineering consortium that is focused on creating better ML for everyone. It aims to accelerate machine learning innovation through benchmarks, public datasets, and best practices. It consists of over 70 supporting organizations from software startups, to researchers at top universities, and to cloud computing and semiconductor giants. In particular, MLCommons builds, maintains, and operates the industry-standard MLPerf benchmark suites. MLCommons follows a holistic approach, with an end-to-end training metric and a very diverse set of benchmarks. It has developed benchmark suites for various scale systems, ranging from mobile devices to the largest supercomputers in the world, aiming to provide fair evaluation and comparison between systems while still encouraging ML innovation. MLCommons has already gone through several rounds of submission on various scale systems, establishing well-defined policies and rules for them with large participation from the industry. MLCommons takes a neutral stand about any form of comparison of results from submissions.

The MLPerf benchmark suites comprise machine learning workloads for training and inference that are representative of production applications including image classification, object detection, and recommendation problems.

MLPerf benchmarks are defined by workloads/reference models, as well as rules, availability classes, and review process. MLPerf Training \cite{mlperf-training} benchmarks aim to measure the performance of training models while MLPerf Inference \cite{mlperf-inference} benchmarks aim to measure how fast systems can process inputs and produce results using a trained model.

\textbf{Relevance:}
The MLPerf HPC benchmarks aim to fill the gaps left by existing benchmark frameworks regarding the ability to characterize performance on large scale systems and remain relevant. These are holistic in the sense that they capture fundamental features of a new class of emerging scientific AI workloads - massive data volume, large complex models, and 

training schemes which incorporate data-parallelism, model-parallelism, and hyper-parameter optimization - making them relevant to industry and academia alike. 
\revision{The MLPerf HPC benchmarks are unique in this sense, offering performance characterization capability for state-of-the-art practices in scientific discovery. Compute intensive simulation workloads are commonplace in HPC environments, requiring massive scale to produce high-impact predictions across a range of scientific domains. Machine learning for science is becoming an important tool to augment and even replace computationally expensive portions of simulation workloads. This coupling between simulation and AI motivates the first two benchmarks included in the suite, Cosmoflow and DeepCAM. Both benchmarks incorporate massive datasets based on simulations and predict important parameters with unprecedented accuracy in their respective domains - cosmology and extreme weather. Future benchmarks for the suite will be community driven, aiming to share similar characteristics with Cosmoflow and DeepCAM while also expanding the relevance of the benchmark suite to other scientific regimes where AI is quickly becoming an important tool for discovery, such as computational biology, materials science and personalized medicine. }
\textbf{Driving Innovation:}
The MLPerf HPC benchmarks drive innovation in system and software design alike - impacting not only machine learning workloads, but the entire set of applications which depend heavily on accelerator devices for fast compute, interconnects for high-bandwidth, low-latency communication, or I/O subsystems that govern the rate at which data can be accessed and moved on multi-user systems.

\textbf{Performance Characterization:}
Additional requirements of the benchmark suite, such as training to convergence, profile generation, and coarse-grained time reporting enable each individual benchmark's performance to be characterized relative to its utilization of a system's I/O, communication, memory, and compute capabilities. This makes the MLPerf HPC Benchmark Suite uniquely capable of characterizing the ability of existing HPC systems to run an exciting class of new workloads, while simultaneously providing engineers a sorely needed standard set of benchmarks for informing the design of tomorrow's large-scale high performance computers.

